DexWeave: Learning Dexterous Humanoid Loco-Manipulation from Human Demonstrations

Learning dexterous humanoid loco-manipulation from human demonstrations requires transferring not only human motion, but also the coordinated interaction structure underlying the demonstrated behavior. This is challenging because embodiment differences distort the coupling among body motion, wrist placement, finger articulation, and object interaction, while kinematically accurate references may still be difficult to realize under robot dynamics. We present DexWeave, a unified framework that connects interaction-consistent motion retargeting with anatomy-aware whole-body policy learning. DexWeave first employs a two-stage retargeting procedure that initializes body and hand motions with specialized solvers and subsequently performs coupled refinement over the upper-body interaction chain while preserving lower-body support. The resulting references are tracked by an anatomy-aware Transformer policy that represents anatomical regions as structured tokens and uses directed masked attention to model their dependencies, with object information selectively conditioning the upper-body pathway for dexterous interaction. The policy jointly outputs body and dexterous-hand actions and is trained directly with reinforcement learning, without pretrained tracking policies, teacher-student distillation, or subsequent residual refinement. DexWeave improves retargeting fidelity and interaction consistency while achieving higher manipulation performance and faster policy convergence than MLP baselines. We further deploy the learned policies on a physical Unitree G1 humanoid equipped with Inspire dexterous hands, demonstrating dexterous whole-body loco-manipulation in the real world. See our project page (https://dexweave.github.io) for videos.

==> src/7_experiments.tex <==
% !TeX root = ../iclr2027_conference.tex
\section{Experiments}\label{sec:experiments}

We evaluate DexWeave's retargeting quality and downstream policy performance for dexterous loco-manipulation. Retargeting experiments assess whole-body feasibility and fine-grained interaction geometry, while policy experiments evaluate closed-loop execution with the anatomy-aware controller. Experiments use a Unitree G1 humanoid equipped with Inspire RH56DFQ dexterous hands. We draw demonstrations from four datasets with different reference information: LAFAN1~\citep{harvey2020robust} contains body-only motions; OMOMO~\citep{li2023object,xu2025intermimic} provides body\textendash{}object interactions without finger references; GRAB~\citep{taheri2020grab} includes articulated hand\textendash{}object interactions; and HUMOTO~\citep{lu2025humoto} contains whole-body activities in cluttered multi-object scenes. All source sequences are resampled to 50\,Hz before retargeting, and the resulting trajectories serve as references for policy learning.

\begin{table}[t]
    \centering
    \caption{
        \textbf{Whole-body retargeting on LAFAN1 and OMOMO.}
        Durations are normalized fractions. Contact metrics apply only to OMOMO; N/A denotes inapplicable entries. \bestvalue{Yellow} and \underline{underlined} values indicate the best and second-best results within each dataset, respectively.
    }\label{tab:retarget_body_contact}

    \footnotesize
    \setlength{\tabcolsep}{4pt}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llcccccc}
        \toprule
        & & \multicolumn{2}{c}{\textbf{Penetration}}
        & \multicolumn{2}{c}{\textbf{Foot Skating}}
        & \multicolumn{2}{c}{\textbf{Contact Preservation}} \\

        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}

        \textbf{Dataset} & \textbf{Method}
        & \shortstack{Duration \\ $\downarrow$}
        & \shortstack{Max Depth \\ (cm) $\downarrow$}
        & \shortstack{Duration \\ $\downarrow$}
        & \shortstack{Max Vel. \\ (cm/s) $\downarrow$}
        & \shortstack{Duration \\ $\uparrow$}
        & \shortstack{Distance \\ (cm) $\downarrow$} \\

        \midrule
        \multirow{4}{*}{\textit{LAFAN1}} & OmniRetarget
        & $\underline{0.125}$ & $\underline{2.934}$
        & 0.091 & $\underline{0.416}$ & N/A & N/A \\

        & GMR
        & 0.183 & 4.314
        & $\underline{0.010}$ & 0.548 & N/A & N/A \\

        & SOMA
        & 0.968 & 6.379
        & 0.115 & 0.565 & N/A & N/A \\

        & DexWeave (Ours)
        & \bestvalue{$0.007$} & \bestvalue{$1.084$}
        & \bestvalue{$0$} & \bestvalue{$0$} & N/A & N/A \\

        \midrule
        \multirow{4}{*}{\textit{OMOMO}} & OmniRetarget
        & $\underline{0.117}$ & $\underline{2.772}$
        & $\underline{\sim{}0}$ & $\underline{0.463}$ & 0.666 & 9.371 \\

        & GMR
        & 0.905 & 3.049
        & 0.007 & 0.805 & $\underline{0.865}$ & $\underline{7.855}$ \\

        & SOMA
        & 0.746 & 4.163
        & 0.034 & 0.467 & 0.577 & 16.205 \\

        & DexWeave (Ours)
        & \bestvalue{$0.003$} & \bestvalue{$2.117$}
        & \bestvalue{$\sim{}0$} & \bestvalue{$0.335$}
        & \bestvalue{$0.999$} & \bestvalue{$2.996$} \\

        \bottomrule
    \end{tabular*}
\end{table}

\subsection{Retargeting Evaluation}

We assess open-loop kinematic quality through whole-body feasibility, hand\textendash{}object alignment, and fine-grained hand geometry. Following the evaluation criteria of OmniRetarget~\citep{yang2025omniretarget}, we compare methods under matched scene conventions and applicable source frames. Duration, distance, and hand-error metrics are averaged equally over applicable sequences. Baseline configurations, metric definitions, geometry backends, thresholds, aggregation rules, and exclusions are detailed in Appendix~\ref{app:retargeting_protocol}.



\paragraph{Whole-body feasibility and contact preservation.}

LAFAN1 and OMOMO evaluate retargeting without finger references. We compare DexWeave with OmniRetarget, GMR~\citep{araujo2025gmr}, and SOMA~\citep{nvidia2026somaretargeter}, measuring penetration and foot skating on both datasets and hand\textendash{}object contact preservation on OMOMO\@.

As shown in Table~\ref{tab:retarget_body_contact}, DexWeave reduces penetration duration on LAFAN1 to 0.007, compared with 0.125 for the best baseline, with no detected foot skating. On OMOMO, it increases contact preservation duration from the best baseline's 0.865 to 0.999 and reduces contact distance from 7.855 to 2.996\,cm. These improvements accompany the lowest penetration duration, 0.003, showing that closer hand\textendash{}object alignment is achieved together with fewer collision artifacts.




\begin{table}[t]
    \centering
    \caption{
        \textbf{Fine-grained interaction retargeting on GRAB and HUMOTO.} + IK corrects hand placement with finger articulation fixed. DexWeave is evaluated before (\emph{decoupled}) and after (\emph{refined}) interaction refinement. Pri. and Sec. Err. measure fingertip position errors for the thumb/index and remaining fingers; Palm Err. measures palm-normal angular error. Penetration duration is a normalized fraction. Foot-skating metrics are omitted because no skating is detected. Within each dataset, yellow highlights and underlined values indicate the best and second-best results across all six methods.
    }
    \label{tab:retarget_dexterous}

    \small
    \setlength{\tabcolsep}{4pt}

    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ll@{\hspace{3pt}}lccccc}
        \toprule
        & & & \multicolumn{2}{c}{\textbf{Penetration}}
        & \multicolumn{3}{c}{\textbf{Hand Alignment}} \\

        \cmidrule(lr){4-5}
        \cmidrule(lr){6-8}

        \textbf{Dataset} & \multicolumn{2}{l}{\textbf{Method}}
        & \shortstack{Duration \\ $\downarrow$}
        & \shortstack{Max Depth \\ (cm) $\downarrow$}
        & \shortstack{Pri. Err. \\ (mm) $\downarrow$}
        & \shortstack{Sec. Err. \\ (mm) $\downarrow$} 
        & \shortstack{Palm Err. \\ (°) $\downarrow$} \\

        \midrule
        \multirow{6}{*}{\textit{GRAB}} & \multirow{4}{*}{OmniRetarget} & + DexPilot
        & $\underline{0.183}$ & 2.123 & 209.353 & 207.745 & 52.122 \\

        & & + DexPilot \textbf{+ IK}
        & 0.212 & 2.269 & 16.585 & \bestvalue{$13.368$} & 11.555 \\

        & & + SBR
        & 0.184 & $\underline{2.120}$ & 210.524 & 212.985 & 52.122 \\

        & & + SBR \textbf{+ IK}
        & 0.190 & 2.362 & $\underline{14.925}$ & 14.659 & 9.530 \\

        & \multirow{2}{*}{DexWeave} & \emph{decoupled}
        & 0.320 & 2.148 & 36.209 & 37.092 & \bestvalue{$0.108$} \\

        & & \emph{\textbf{refined}}
        & \bestvalue{$0.001$} & \bestvalue{$1.378$} & \bestvalue{$4.158$} & $\underline{14.212}$ & $\underline{3.282}$ \\

        \midrule
        \multirow{6}{*}{\textit{HUMOTO}} & \multirow{4}{*}{OmniRetarget} & + DexPilot
        & 0.370 & 3.638 & 292.886 & 278.574 & 47.815 \\

        & & + DexPilot \textbf{+ IK}
        & 0.522 & 3.597 & 32.389 & 31.018 & 14.444 \\

        & & + SBR
        & 0.370 & 3.638 & 292.750 & 283.381 & 47.815 \\

        & & + SBR \textbf{+ IK}
        & 0.511 & 3.582 & $\underline{29.999}$ & 28.436 & 12.476 \\

        & \multirow{2}{*}{DexWeave} & \emph{decoupled}
        & $\underline{0.267}$ & $\underline{2.847}$ & 32.791 & $\underline{26.204}$ & \bestvalue{$0.096$} \\

        & & \emph{\textbf{refined}}
        & \bestvalue{$0.004$} & \bestvalue{$2.585$} & \bestvalue{$6.382$} & \bestvalue{$11.454$} & $\underline{3.794}$ \\

        \bottomrule
    \end{tabular*}
\end{table}


\paragraph{Fine-grained interaction retargeting.}
On GRAB and HUMOTO, we compare DexWeave with OmniRetarget paired with DexPilot~\citep{handa2020dexpilot} or the Sampling-Based Retargeter (SBR)~\citep{malate2026smoothoperator}. Each baseline is evaluated with and without arm--wrist IK, which corrects hand placement while fixing finger articulation. The IK variants test whether joint refinement offers improvements beyond placement correction alone. Comparing DexWeave's decoupled initialization with its refined output isolates the refinement contribution.

Table~\ref{tab:retarget_dexterous} shows that our decoupled initialization yields lower fingertip and palm-normal errors than direct combinations of OmniRetarget with DexPilot or SBR. This supports our wrist-target design for aligning body and hand motions. Full DexWeave further achieves lower penetration and primary fingertip errors than the IK-corrected baselines on both datasets.

Relative to the decoupled initialization, refinement reduces primary fingertip errors by 88.5\% on GRAB and 80.5\% on HUMOTO, while also decreasing penetration. Meanwhile, palm-normal errors increase from approximately $0.1^\circ$ to $3.282^\circ$ and $3.794^\circ$, respectively. This difference arises because the initialization primarily preserves wrist and palm orientations, whereas refinement jointly optimizes the upper-limb interaction chain to better accommodate human–robot hand embodiment differences. The resulting slight deviation in palm orientation improves the overall hand–object geometric alignment.

Figure~\ref{fig:retargeting_results} shows these refined hand--object configurations within whole-body motions, pairing sequence overviews with interaction close-ups across four examples. We next evaluate closed-loop loco-manipulation using policies trained on the refined references.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/loco_manip_retarget.pdf}
    \caption{
        \textbf{DexWeave retargeting results.}
        Four retargeted sequences pair whole-body motion snapshots
        with enlarged views of the corresponding hand\textendash{}object
        configurations. The close-ups show local interaction geometry
        within each whole-body motion.
    }\label{fig:retargeting_results}
\end{figure}


\subsection{Policy Evaluation}\label{sec:policy_experiments}

We evaluate the anatomy-aware actor in closed-loop dexterous loco-manipulation, with body-only motion tracking as an auxiliary setting. All policies output 41-dimensional joint-position targets and are trained with PPO (Sec.~\ref{sec:ppo_training}). For each actor configuration, we train a separate policy on each of five retargeted reference sequences drawn from the evaluated datasets. Reported metrics are arithmetic means of the five sequence-level results. Within each actor comparison, we hold the references, observation information, action space, rewards, critic, reset and termination rules, domain randomization, and environment-interaction budget fixed. This protocol compares actor architectures under a shared control setup. Sequence identities, training settings, and evaluation definitions are provided in Appendix~\ref{app:policy_protocol}.

\paragraph{Dexterous loco-manipulation.}

Our main evaluation considers tasks that combine body displacement with dexterous hand\textendash{}object interaction. We compare DexWeave with an object-conditioned MLP using the same refined references and robot and object observations. Both actors jointly learn whole-body tracking and object interaction within a single PPO stage. DexWeave augments its body-token backbone with an object token and task-aware attention, allowing the same architecture to support object-conditioned control. Table~\ref{tab:policy_locomanipulation} evaluates task success and object-pose accuracy together with body tracking error and fall rate. These complementary metrics assess interaction execution, motion fidelity, and postural stability within the same tasks.

\begin{table}[t]
    \centering
    \caption{
        \textbf{Dexterous loco-manipulation in simulation.}
        Actors share refined references, observation information,
        and PPO settings. Success and object-pose errors assess
        interaction performance; body error and fall rate assess
        whole-body execution. Results are averaged over five
        sequence-level evaluations. Task-specific success criteria
        and metric definitions are given in
        Appendix~\ref{app:policy_protocol}.
        Dashes denote unreported results.
    }\label{tab:policy_locomanipulation}

    \small
    \setlength{\tabcolsep}{3pt}

    \begin{tabular}{@{}lccccc@{}}
        \toprule
        \textbf{Actor}
        & \shortstack{Success\\(\%) $\uparrow$}
        & \shortstack{Object pos.\\(cm) $\downarrow$}
        & \shortstack{Object rot.\\(deg) $\downarrow$}
        & \shortstack{Body error\\(cm) $\downarrow$}
        & \shortstack{Falls\\(\%) $\downarrow$} \\

        \midrule
        Object-conditioned MLP
        & \textendash{} & \textendash{} & \textendash{} & \textendash{} & \textendash{} \\

        DexWeave (Transformer)
        & \textendash{} & \textendash{} & \textendash{} & \textendash{} & \textendash{} \\

        \bottomrule
    \end{tabular}
\end{table}

\FloatBarrier{}

\paragraph{Motion tracking.}

To assess the shared actor design without object conditioning, we compare DexWeave with an MLP actor adapted from the tracking component of BeyondMimic~\citep{liao2025beyondmimic}. Full-reference completion measures execution reliability, while root-relative body error and global root error measure pose and trajectory accuracy (Table~\ref{tab:policy_tracking}). Figure~\ref{fig:policy_learning} plots completion against environment interactions and elapsed training time to distinguish sample efficiency from training time, alongside representative time-aligned reference and robot poses.

\begin{table}[!htb]
    \centering
    \caption{
        \textbf{Body-only motion tracking.}
        BeyondMimic denotes its MLP tracking actor adapted to the
        shared robot and observations. Body error uses root-relative
        body positions; root error uses the global root position.
        Results are averaged over five sequence-level evaluations
        at the matched interaction budget.
        Dashes denote unreported results.
    }\label{tab:policy_tracking}

    \small
    \setlength{\tabcolsep}{8pt}

    \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Actor}
        & \shortstack{Completion\\(\%) $\uparrow$}
        & \shortstack{Body error\\(cm) $\downarrow$}
        & \shortstack{Root error\\(cm) $\downarrow$} \\

        \midrule
        BeyondMimic (MLP)
        & \textendash{} & \textendash{} & \textendash{} \\

        DexWeave (Transformer)
        & \textendash{} & \textendash{} & \textendash{} \\

        \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[!htb]
    \centering
    \figplaceholder{0.49\linewidth}{1.55cm}{\textbf{(a) Sample efficiency}\\Tracking completion vs.\ environment interactions} \hfill
    \figplaceholder{0.49\linewidth}{1.55cm}{\textbf{(b) Training time}\\Tracking completion vs.\ elapsed time}\\[4pt]
    \figplaceholder{\linewidth}{1.55cm}{\textbf{(c) Motion-tracking execution}\\Time-aligned reference and robot poses}
    \caption{
        \textbf{Motion-tracking policy evaluation.}
        Full-reference completion for MLP and Transformer actors
        against (a) environment interactions and (b) elapsed training
        time, averaged over five reference sequences;
        (c) time-aligned reference and robot poses for representative
        body motions.
    }\label{fig:policy_learning}
\end{figure}

\FloatBarrier{}

\paragraph{Hardware evaluation.}

We assess physical deployment on the G1 with Inspire hands using dexterous loco-manipulation tasks. Figure~\ref{fig:execution_results} presents whole-body sequences and corresponding hand\textendash{}object close-ups in simulation and on hardware. Hardware evaluation uses successful trials out of attempted trials for each task, with observed failure modes analyzed separately from simulation metrics. Sensing, deployment settings, trial outcomes, and failure descriptions are provided in Appendix~\ref{app:hardware_protocol}.

\begin{figure}[!htb]
    \centering
    \figplaceholder{\linewidth}{1.7cm}{\textbf{(a) Simulation}\\Whole-body sequence and hand\textendash{}object close-ups}\\[4pt]
    \figplaceholder{\linewidth}{1.7cm}{\textbf{(b) Physical G1 with Inspire hands}\\Whole-body sequence and hand\textendash{}object close-ups}
    \caption{
        \textbf{Dexterous loco-manipulation execution.}
        Whole-body motion sequences with corresponding hand\textendash{}object
        close-ups in (a) simulation and (b) physical G1 deployment
        with Inspire hands. The views show body motion and local
        interaction geometry at corresponding task phases.
    }\label{fig:execution_results}
\end{figure}

\FloatBarrier{}

